A stability barrier for reconstructions from Fourier samples

We prove that any stable method for resolving the Gibbs phenomenon - that is, recovering high-order accuracy from the first $m$ Fourier coefficients of an analytic and nonperiodic function - can converge at best root-exponentially fast in $m$. Any method with faster convergence must also be unstable, and in particular, exponential convergence implies exponential ill-conditioning. This result is analogous to a recent theorem of Platte, Trefethen & Kuijlaars concerning recovery from pointwise function values on an equispaced $m$-grid. The main step in our proof is an estimate for the maximal behaviour of a polynomial of degree $n$ with bounded $m$-term Fourier series, which is related to a conjecture of Hrycak & Groechenig. In the second part of the paper we discuss the implications of our main theorem to polynomial-based interpolation and least-squares approaches for overcoming the Gibbs phenomenon. Finally, we consider the use of so-called Fourier extensions as an attractive alternative for this problem. We present numerical results demonstrating rapid convergence in a stable manner.

==> def2 <==
\renewcommand{\arraystretch}{1.5}

%\font\sBbb=msbm7 scaled 1000
%\font\gothic=eufm10 scaled 1100
%\font\smallgothic=eufm7 scaled 1100

%\def\bb#1{\mbox{\sBbb #1}}             % Shell capitals in subscript
%\def\CC#1{\mathrm{#1}}                 % Roman
%\def\Gg#1{\mbox{\smallgothic #1}}      % Gothic in subscript
%\def\GG#1{\mbox{\gothic #1}}           % Gothic

\def \Mm#1{\mbox{\boldmath$\scriptstyle #1$\unboldmath}}
                                       % Math-bold in subscript 
\def \MM#1{\mbox{\boldmath$#1$\unboldmath}}
\font\Bbb=msbm10 scaled 1000
\def\BB#1{\mbox{\Bbb #1}}              % Shell capitals
\font\sBbb=msbm7 scaled 1000
\def\Bb#1{\mbox{\sBbb #1}}             % Shell capitals in subscript

\newcommand {\by} {{{\boldmath$y$\unboldmath}}}
\newcommand {\bx} {{\boldmath$x$\unboldmath}}
\def \x {{\Mm{x}}}
\def \y {{\Mm{y}}}
\def \h {\Mm{h}}
\def \xx {\MM{x}}
\def \yy {\MM{y}}
\def \ii {\MM{i}}
\def \jj {\MM{j}}
\def \hh {\MM{h}}

\def\Frac#1#2{\mbox{\large${\textstyle \frac{#1}{#2}}$}}
%\def\Frac#1#2{{\textstyle \frac{#1}{#2}}}

\def \p {{\partial}}
\def \ub {\underbrace}


\def \R  {{\mathbb{R}}}
\def \Rnn {\R^{n\times n}}
\def \L {{L_2(\R)}}
\def \rn  {{\Bb{R}^n}}
\def \C   {{\mathbb{C}}}
\def \X   {{\mathbb{X}}}
\def \N   {{\mathbb{N}}}
\def \F   {{\BB{F}}}
%\def \N   {{\BB{N}}}
%\def \T   {{\BB{T}}}
\def \T   {{\mathbb{T}}}
\def \Y   {{\mathbb{Y}}}
\def \Z   {{\mathbb{Z}}}

\def \PP {{\cal P}}
\def \AA {{\cal A}}
\def \SS {{\cal S}}
\def \LL {{\cal L}}
\def \FF {{\cal F}}
\def \OO {{\cal O}}
\def \TT {{\cal T}}
\def \ZZ {{\cal Z}}
\def \CC {{\cal C}}
\def \UU {{\cal U}}


\def \al  {\alpha}
\def \e {\varepsilon}
\def \Om  {\Omega}
\def \la  {\lambda}
\def \de  {\delta}
\def \ga  {\gamma}
\def \De  {\Delta}


\def\l {\ell}

\def \lr {{\quad\Leftrightarrow\quad}}
\def \ra {{\quad\Rightarrow\quad}}
\def \wt {\widetilde}
\def \wh {\widehat}



\def\be {\begin{equation}}
\def\ee {\end{equation}}
\def\ba {\begin{eqnarray}}
\def\ea {\end{eqnarray}}
\def\baa {\begin{eqnarray*}}
\def\eaa {\end{eqnarray*}}

\newcommand{\sm}{{\setminus}}


\def \spa {{\rm span}}
\def \rank {{\rm rank}}
\def \sign {{\rm sgn\,}}
\newcommand{\mes}{{\rm mes\,}}
\newcommand{\dist}{{\rm dist}}
\newcommand{\const}{{\rm const}}
\newcommand{\Lip}{{\rm Lip}}
\newcommand{\supp}{{\rm supp\,}}
\newcommand{\diag}{{\rm diag\,}}


\newcommand{\on}{\quad\mbox{on}\quad}
\newcommand{\ifi}{\quad\mbox{if}\quad}
\newcommand{\at}{\quad\mbox{at}\quad}
\newcommand{\for}{\quad\mbox{for}\;}
\newcommand{\all}{\quad\mbox{all}\;}
\newcommand{\where}{\quad\mbox{where}\quad}
\newcommand{\with}{\quad\mbox{with}\quad}
\newcommand{\an}{\quad\mbox{and}\quad}


%
\def\proof{\noindent{\bf Proof.} }
\def\qed{\hfill $\Box$}
%\def\qed{\hfill \rule{1.5mm}{1.5mm}}
%\def\qed{\raisebox{1mm}{\fbox{\rule{0mm}{0mm}}}}
%
\newcommand {\lb} {\label}
\newcommand {\rf[1]} {(\ref{#1})}




